An Examination of the Robustness of Reference-Free Image Captioning Evaluation Metrics

Recently, reference-free metrics such as CLIPScore (Hessel et al., 2021), UMIC (Lee et al., 2021), and PAC-S (Sarto et al., 2023) have been proposed for automatic reference-free evaluation of image captions. Our focus lies in evaluating the robustness of these metrics in scenarios that require distinguishing between two captions with high lexical overlap but very different meanings. Our findings reveal that despite their high correlation with human judgments, CLIPScore, UMIC, and PAC-S struggle to identify fine-grained errors. While all metrics exhibit strong sensitivity to visual grounding errors, their sensitivity to caption implausibility errors is limited. Furthermore, we found that all metrics are sensitive to variations in the size of image-relevant objects mentioned in the caption, while CLIPScore and PAC-S are also sensitive to the number of mentions of image-relevant objects in the caption. Regarding linguistic aspects of a caption, all metrics show weak comprehension of negation, and CLIPScore and PAC-S are insensitive to the structure of the caption to a great extent. We hope our findings will guide further improvements in reference-free evaluation of image captioning.

==> sections/experiments/6-length.tex <==
% In this section, our objective is to evaluate the sensitivity of CLIPScore and UMIC to sentence length rather than correctness. To accomplish this, we first filtered out the incorrect answers generated by ALBEF on the TDIUC validation set and we generated caption-like sentences for them. Additionally, we generated a caption-like sentence based on the question only by utilizing GPT-J in a few-shot manner (see Figure \ref{fig:ref_gen}). As a result, these question-based sentences are shorter than the sentences generated using both questions and answers. In terms of performance evaluation, for CLIPScore, longer caption-like sentences with incorrect answers received an average score of $0.521 \pm 0.129$, while question-based captions received an average score of $0.512 \pm 0.116$. On the other hand, UMIC assigned a higher score of $0.351 \pm 0.196$ to longer caption-like sentences with incorrect answers, while shorter question-based captions received an average score of $0.264 \pm 0.149$. In total, for CLIPScore, 53.16\% of the time, the score of question-based captions was lower than that of captions with incorrect answers, and for UMIC, 62.08\% of the time. In conclusion, \textbf{UMIC exhibits significant sensitivity to caption length while CLIPScore exhibits limited sensitivity}.
% To evaluate the sensitivity of CLIPScore and UMIC to sentence length rather than correctness, we first filtered out the incorrect answers generated by ALBEF on the TDIUC validation set and we generated caption-like sentences for them. Additionally, we generated a caption-like sentence based on the question only by utilizing GPT-J in a few-shot manner (see Figure \ref{fig:ref_gen}). As a result, these question-based sentences are shorter than the sentences generated using both questions and answers. In terms of performance evaluation, for CLIPScore, longer caption-like sentences with incorrect answers received an average score of $0.521 \pm 0.129$, while question-based captions received an average score of $0.512 \pm 0.116$. On the other hand, UMIC assigned a higher score of $0.351 \pm 0.196$ to longer caption-like sentences with incorrect answers, while shorter question-based captions received an average score of $0.264 \pm 0.149$.  In conclusion, \textbf{UMIC exhibits significant sensitivity to caption length while CLIPScore exhibits limited sensitivity}.
To evaluate whether the metrics are more sensitive to the sentence length rather than the correctness of the sentence, we first filtered out the incorrect answers generated by ALBEF on the TDIUC validation set, and we generated 49385 caption-like sentences for them. Additionally, we generated a caption-like sentence based on the question only by utilizing GPT-J in a few-shot manner (see Appendix \ref{fig:ref_gen} for a visualization). As a result, these question-based sentences are shorter than the sentences generated using both questions and answers but are correct sentences. We observed that for CLIPScore, longer caption-like sentences with incorrect answers received an average score of $0.521$, while question-based captions received an average score of $0.512$. On the other hand, UMIC assigned a higher score of $0.351$ to longer caption-like sentences with incorrect answers, while shorter question-based captions received an average score of $0.264$. When we look at the ranking results, for CLIPScore, 53.16\% of the time, the scores of question-based captions were lower than that of captions with incorrect answers, and for UMIC, 62.08\% of the time. In conclusion, \textbf{UMIC exhibits significant sensitivity to caption length while CLIPScore exhibits limited sensitivity}.


==> tables/caption_length.tex <==
\begin{table}
    \centering
        {\begin{tabular}{lcc}
            \hline
            \textbf{Answer Type} & \textbf{CLIPScore} & \textbf{UMIC}\\
            \hline
            Shorter but Correct &  $0.512$ & $0.264$\\
            Longer but Incorrect & $0.521$& $0.351$\\ \hline
        \end{tabular}}
    \caption{CLIPScore and UMIC comparison for correct and incorrect negated version of caption.}
    \label{tab:length}
\end{table}


==> tables/clipscore_umic_tdiuc_question_types.tex <==
\begin{table*}[t]
    \centering
    % \resizebox{\textwidth}{!}
        {\begin{tabular}{lcccc}
            \hline
            % \textbf{\textit{Question Type}} & \textbf{\textit{CLIPScore-Incorrect}} & \textbf{\textit{CLIPScore-Correct}} & \textbf{\textit{UMIC-Incorrect}} & \textbf{\textit{UMIC-Correct}}\\
            \textbf{\textit{Question}} & \textbf{\textit{CLIPScore}} & \textbf{\textit{CLIPScore}} & \textbf{\textit{UMIC}} & \textbf{\textit{UMIC}}\\
            \textbf{\textit{\;\;\;Type}} & \textbf{\textit{Incorrect}} & \textbf{\textit{Correct}} & \textbf{\textit{Incorrect}} & \textbf{\textit{Correct}}\\
            \hline
            absurd  &  $0.422$ & $ 0.388$  &  $ 0.096$ & $ 0.011$ \\
            attribute  &  $0.550$ & $ 0.546$   &  $ 0.428$ & $ 0.458$ \\
            color  &  $ 0.542$ & $ 0.551$ &  $ 0.439$ & $ 0.498$\\
            object presence  &  $ 0.500$ & $ 0.492$ &  $ 0.179$ & $ 0.188$ \\
            sport recognition  &  $ 0.597$ & $ 0.667$  &  $ 0.253$ & $ 0.326$ \\
            activity recognition  &  $ 0.645$ & $ 0.664$ &  $ 0.353$ & $ 0.390$ \\
            sentiment understanding  &  $ 0.582$ & $ 0.564$ &  $ 0.4098 $ & $ 0.421$ \\
            scene recognition  &  $ 0.497$ & $ 0.513$  &  $ 0.264$ & $ 0.182$ \\
            utility affordance  &  $ 0.562$ & $ 0.591$  &  $ 0.353$ & $ 0.353$ \\
            positional reasoning  &  $ 0.613$ & $ 0.638$ &  $ 0.425$ & $ 0.504$ \\
            counting  &  $ 0.563$ & $ 0.572$  &  $ 0.300$ & $ 0.339$ \\
            object recognition  &  $ 0.554$ & $ 0.595$  &  $ 0.251 $ & $ 0.284$ \\ \hline
    \end{tabular}}
    \caption{CLIPScore and UMIC score for correct and incorrect caption-like sentences generated for different question types of TDIUC.}
    \label{tab:clipscore_umic_tdiuc_question_types}
\end{table*}


% \begin{table}
%   \caption{CLIPScore and UMIC score for correct and incorrect caption-like sentences generated for different question types of TDIUC.}
% \label{tab:clipscore_umic_tdiuc_question_types}
%   \centering
%   \resizebox{\textwidth}{!}
%     {
%   \begin{tabular}{lllll}
%     \toprule
%     \textbf{\textit{Question Type}} & \textbf{\textit{CLIPScore-Incorrect}} & \textbf{\textit{CLIPScore-Correct}} & \textbf{\textit{UMIC-Incorrect}} & \textbf{\textit{UMIC-Correct}} \\
%     \midrule
%     absurd  &  $0.422$ & $ 0.388$  &  $ 0.096$ & $ 0.011$ \\
%     attribute  &  $0.550$ & $ 0.546$   &  $ 0.428$ & $ 0.458$ \\
%     color  &  $ 0.542$ & $ 0.551$ &  $ 0.439$ & $ 0.498$\\
%     object presence  &  $ 0.500$ & $ 0.492$ &  $ 0.179$ & $ 0.188$ \\
%     sport recognition  &  $ 0.597$ & $ 0.667$  &  $ 0.253$ & $ 0.326$ \\
%     activity recognition  &  $ 0.645$ & $ 0.664$ &  $ 0.353$ & $ 0.390$ \\
%     sentiment understanding  &  $ 0.582$ & $ 0.564$ &  $ 0.4098 $ & $ 0.421$ \\
%     scene recognition  &  $ 0.497$ & $ 0.513$  &  $ 0.264$ & $ 0.182$ \\
%     utility affordance  &  $ 0.562$ & $ 0.591$  &  $ 0.353$ & $ 0.353$ \\
%     positional reasoning  &  $ 0.613$ & $ 0.638$ &  $ 0.425$ & $ 0.504$ \\
%     counting  &  $ 0.563$ & $ 0.572$  &  $ 0.300$ & $ 0.339$ \\
%     object recognition  &  $ 0.554$ & $ 0.595$  &  $ 0.251 $ & $ 0.284$ \\
%     \bottomrule
%   \end{tabular}}
% \end{table}


% clipscore
% incorrect_rank 4 ['absurd', 'attribute', 'object_presence', 'sentiment_understanding']
% overlap 12 ['absurd', 'attribute', 'color', 'object_presence', 'sport_recognition', 'activity_recognition', 'sentiment_understanding', 'scene_recognition', 'utility_affordance', 'positional_reasoning', 'counting', 'object_recognition']

% umic
% incorrect_rank 3 ['utility_affordance', 'absurd', 'scene_recognition']
% overlap 12 ['counting', 'positional_reasoning', 'object_recognition', 'utility_affordance', 'sport_recognition', 'activity_recognition', 'object_presence', 'absurd', 'sentiment_understanding', 'color', 'attribute', 'scene_recognition']


==> tables/negation.tex <==
% \begin{table}
%     \centering
%         {\begin{tabular}{lcc}
%             \hline
%             \textbf{Answer Type} & \textbf{CLIPScore} & \textbf{UMIC}\\
%             \hline
%             Correct &  $0.457$ & $0.359$\\
%             Incorrect by negation & $0.450$& $0.335$\\ \hline
%         \end{tabular}}
%     \caption{CLIPScore and UMIC comparison for correct and incorrect negated version of caption.}
%     \label{tab:negation}
% \end{table}
\begin{table}
    \centering
        {\begin{tabular}{lccc}
            \hline
            \textbf{Answer Type} & \textbf{CLIPScore} & \textbf{UMIC} & \textbf{PAC-S} \\
            \hline
            Correct &  $0.457$ & $0.359$ &  0.$556$\\
            Incorrect by negation & $0.450$& $0.335$ & $0.548$\\ \hline
        \end{tabular}}
    \caption{CLIPScore and UMIC comparison for correct and incorrect negated version of caption.}
    \label{tab:negation}
\end{table}
% min, max:  0.37421977519989014 0.9781562089920044
% correct 0.5563199128284984 0.1250570170011364
% negated 0.5488316838579301 0.12799441634170153
% len all_scores 80530
% almost_equal_correct 1.277737076726311 %
% incorrect_ranking 41.83626587858393
% t-test correct_scores/incorrect_scores:  Ttest_indResult(statistic=11.874961426286417, pvalue=1.6478307212740136e-32)

==> tables/perplexity.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{\linewidth}{!}
        {\begin{tabular}{lcccccccc}
            \hline
            % \textbf{COCO Caption} & \textbf{COCO Caption} & \textbf{COCO Caption} & \textbf{COCO Caption} & \textbf{COCO Caption} & \textbf{COCO Caption} & \textbf{QA to Caption Conversion} & \textbf{QA to Caption Conversion}\\
            \textbf{Caption Set} & \textbf{COCO Set 1} & \textbf{COCO Set 2} & \textbf{COCO Set 3} & \textbf{COCO Set 4} & \textbf{COCO Set 5} & \textbf{Incorrect Caption-like} & \textbf{Correct Caption like}  & \textbf{Caption Template}\\ \hline
            \textbf{Perplexity} & $73.76$  & $78.80$  & $82.32$  & $80.26$  & $77.02$  & $164.41$  & $160.77$ & $55.69$ \\ \hline
        \end{tabular}}
    \caption{The perplexity (under the GPT-3 model) of COCO human written captions, incorrect and correct caption-like sentences generated using the QA to caption conversion method, and the captions generated using the caption template method.}
    \label{tab:perplexity}
\end{table*}
% \begin{table}
%     \centering
%     \resizebox{\linewidth}{!}
%         {\begin{tabular}{lcccccccc}
%             \hline
%             \textbf{COCO Caption} & \textbf{COCO Caption} & \textbf{COCO Caption} & \textbf{COCO Caption} & \textbf{COCO Caption} & \textbf{COCO Caption} & \textbf{QA to Caption Conversion} & \textbf{QA to Caption Conversion}\\
%             \textbf{Set 1} & \textbf{Set 2} & \textbf{Set 3} & \textbf{Set 4} & \textbf{Set 5} & & \textbf{} & \textbf{Incorrect} & \textbf{Correct}\\ \hline
%             Perplexity & $73.76$  & $78.80$  & $82.32$  & $80.26$  & $77.02$  & $55.69$  & $164.41$  & $160.77$\\ \hline
%         \end{tabular}}
%     \caption{Perplexity of COCO human written captions, captions generated using caption templates and incorrect and correct caption-like sentences using QA to caption conversion method.}
%     \label{tab:perplexity}
% \end{table}
% caption_template PPl 55.69832806926413
% QA_incorrect_captions PPl 164.4136500880542
% QA_correct_captions PPl 160.7782245686484
% sample_set0 PPl 73.76674402907855
% sample_set1 PPl 78.80625486556484
% sample_set2 PPl 82.32235583037452
% sample_set3 PPl 80.26157717352055
% sample_set4 PPl 77.02708755776987

==> tables/vqa_sentence_structure.tex <==
% \begin{table}
%     \centering
%     \resizebox{\linewidth}{!}
%         {\begin{tabular}{lcc}
%             \hline
%             \textbf{Answer Type} & \textbf{CLIPScore} & \textbf{UMIC}\\
%             \hline
%             Correct answer &  $0.469$ & $0.400$\\
%             Shuffled version & $0.450$ & $0.211$\\ \hline
%         \end{tabular}}
%     \caption{CLIPScore and UMIC comparison for captions generated with ground truth answers of VQAv2 and their shuffled counterparts.}
%     \label{tab:vqa_sentence_structure}
% \end{table}
\begin{table}
    \centering
    \resizebox{\linewidth}{!}
        {\begin{tabular}{lccc}
            \hline
            \textbf{Answer Type} & \textbf{CLIPScore} & \textbf{UMIC} & \textbf{PAC-S}\\
            \hline
            Correct answer &  $0.469$ & $0.400$ & $0.548$\\
            Shuffled version & $0.450$ & $0.211$ & $0.539$\\ \hline
        \end{tabular}}
    \caption{CLIPScore, UMIC and PAC-S comparison for captions generated with ground truth answers of VQAv2 and their shuffled counterparts.}
    \label{tab:vqa_sentence_structure}
\end{table}

% min, max:  0.35105249285697937 1.0224053859710693
% correct 0.5489593984755164 0.11792024263073518
% shuffled 0.5393319114562908 0.11747901494549334
% t-test correct_short/incorrect_long:  Ttest_indResult(statistic=26.778538513327884, pvalue=7.759888832788743e-158)
% len all_scores 214354
% almost_equal_correct 0.029390634184573182 %
% incorrect_ranking 43.05727908039971
